LoRa Backscatter Communications: Temporal, Spectral, and Error Performance Analysis

LoRa backscatter (LB) communication systems can be considered as a potential candidate for ultra low power wide area networks (LPWAN) because of their low cost and low power consumption. In this paper, we comprehensively analyze LB modulation from various aspects, i.e., temporal, spectral, and error performance characteristics. First, we propose a signal model for LB signals that accounts for the limited number of loads in the tag. Then, we investigate the spectral properties of LB signals, obtaining a closed-form expression for the power spectrum. Finally, we derived the symbol error rate (SER) of LB with two decoders, i.e., the maximum likelihood (ML) and fast Fourier transform (FFT) decoders, in both additive white Gaussian noise (AWGN) and double Nakagami-m fading channels. The spectral analysis shows that out-of-band emissions for LB satisfy the European Telecommunications Standards Institute (ETSI) regulation only when considering a relatively large number of loads. For the error performance, unlike conventional LoRa, the FFT decoder is not optimal. Nevertheless, the ML decoder can achieve a performance similar to conventional LoRa with a moderate number of loads.

==> Figures/Figure1/Figure1.tex <==
\pgfplotsset{every axis/.append style={
		font=\footnotesize,
		line width=1pt,
		legend style={font=\footnotesize, at={(0.98,0.31)}},legend cell align=left},
	% 	legend style={font=\footnotesize, at={(0.99,0.75)}}
} %
\pgfplotsset{compat=1.13}
	\begin{tikzpicture}%[trim axis right]%[trim axis left, trim axis right]
\begin{axis}[
%axis
%loglog
%title=Exact Analysis of WCL,
%axis x line=bottom,
%yticklabel style = {font=\footnotesize,xshift=0.5ex},
%xticklabel style = {font=\footnotesize,yshift=0.5ex},
%ylabel style = {font=\huge},
%xlabel style = {font=\huge},
xlabel near ticks,
ylabel near ticks,
grid=major,
xlabel={$X$ (m)},
ylabel={$Y$ (m)},
width=0.99\linewidth,%3.5in,
%	ytick={10,0,-10,-20,-30,-40},
%	x label style={at={(axis description cs:0.5,-0.07)},anchor=north},
%   y label style={at={(axis description cs:-0.11,.5)},rotate=0,anchor=south},
yticklabel style={/pgf/number format},
%axis y line=left,
width=0.99\linewidth,
%height=0.6\textwidth,
%	legend columns=1,	
legend entries={firstmethos \cite{ElzGioChi:19}
	,second $\x$,
	third},
% 	log ticks with fixed point, 
%	scale only axis,
%	restrict
%	xmin= 5, xmax=35,
%	ymin=0.5e-5, ymax=1e1,
ylabel style={font=\Large},
xlabel style={font=\Large},
%minor y tick num=10,
]
\addplot[blue,dashed,mark=star] table {Figures/Figure1/BERM2methodfirstapproach.dat};
\addplot[orange!20!brown,mark=diamond,dashed] table {Figures/Figure1/BERM2methodsecondapproach.dat};
\addplot[black,mark=o,dashed,mark options=solid] table {Figures/Figure1/BERM2methodthirdapproach.dat};
%	\addplot[red,dashed,mark=square] table {crbNoLISa4.dat};

%		\addplot[blue,mark=star] table {crbLISa1.dat};
%	\addplot[orange!20!brown ,mark=diamond,mark repeat=1] table {crbLISa2.dat};
%	\addplot[black,mark=o,mark options=solid] table {crbLISa3.dat};
% 	\addplot[red,mark=square] table {crbLISa4.dat};
%	\addplot[red,mark=square,mark repeat=4,dashed,mark options=solid] table {TSBCIM4fadingM4.dat};
%	\addplot[orange,mark=triangle,mark options=solid,mark repeat=2] table {UniformSD5fadingM4.dat}; 
%\addplot[orange,mark=star,mark size=1.5,mark repeat=6] table {UniformBCIM6fadingM4.dat};
%\addplot[brown] table {CapacityLBfadingM4.dat};
%\addplot[gray] table {PSDCEXPSF7.dat};
%\addplot[black,thick,mark repeat=4,mark options=solid] table {TxRatefadingM4.dat};
%\addplot[gray!50!black,thick,mark=o,mark options=solid, mark size=3] coordinates {
%	(6.65,1.13)
%};

%\addplot[gray,thin] table {Figures/FigPSDContMatlab/FFTFigPSDContSF12.txt};
%%/tikz/thin (no value)
%/tikz/ultra thin (no value)
%/tikz/very thin (no value)
%/tikz/semithick (no value)
%/tikz/thick (no value)
%/tikz/very thick (no value)
%/tikz/ultra thick
\end{axis}
\end{tikzpicture}

==> Figures/PSD/TheoreticalVsWelch/Figure_TheoreticalVsWelch.tex <==
\pgfplotsset{every axis/.append style={
		font=\footnotesize,
		line width=1pt,
		legend style={font=\footnotesize, at={(0.99,0.99)}},legend cell align=left,nodes={scale=0.7, transform shape}},
	% 	legend style={font=\footnotesize, at={(0.99,0.75)}}
} %
\pgfplotsset{compat=1.13}
	\begin{tikzpicture}%[trim axis right]%[trim axis left, trim axis right]
\begin{axis}[
%ymode=log,
%axis
%loglog
%title=Exact Analysis of WCL,
%axis x line=bottom,
%yticklabel style = {font=\footnotesize,xshift=0.5ex},
%xticklabel style = {font=\footnotesize,yshift=0.5ex},
%ylabel style = {font=\huge},
%xlabel style = {font=\huge},
xlabel near ticks,
ylabel near ticks,
grid=both,%major,minor,both,none
xlabel={$f/B$},
ylabel={Power Spectrum (dB)},
%width=0.99\linewidth,%3.5in,
	ytick={5,0,-5,-10,-15,-20,-25,-30,-35},
%	x label style={at={(axis description cs:0.5,-0.07)},anchor=north},
%   y label style={at={(axis description cs:-0.11,.5)},rotate=0,anchor=south},
yticklabel style={/pgf/number format},
%axis y line=left,
width=0.99\linewidth,
%height=0.6\textwidth,
%	legend columns=3,	
%legend pos=south west
%legend entries={
%	$r_\mathrm{t}=1$ \ MC,
%	$r_\mathrm{t}=1$ \ App,
%	$r_\mathrm{t}=4$ \ Num,
%	$r_\mathrm{t}=4$ \ MC,
%	$r_\mathrm{t}=4$ \ App,
%	$r_\mathrm{t}=16$ Num,
%	$r_\mathrm{t}=16$ MC,
%	$r_\mathrm{t}=16$ App
%	},
% 	log ticks with fixed point, 
%	scale only axis,
%	restrict
	xmin= 0, xmax=2,
	ymin=-25, ymax=5,
ylabel style={font=\Large},
xlabel style={font=\Large},
%minor y tick num=10,
]
%\node[anchor=west] (source) at (axis cs:18,7e-1){Tag moving closer to Tx/Rx};
%\node (destination) at (axis cs:12,1e-3){};
%\draw[->](source)--(destination);
%\addplot[blue!60!white,solid] table {Figures/fading_distance/SERNumMLr1.dat};
%\addlegendentry{$r_\mathrm{t}=1$ \ Num}
\addplot[blue!70!white]table {Figures/PSD/TheoreticalVsWelch/PSDataSF7NQ2.dat};
\addlegendentry{Theoretical};



\addplot[red!70!white,only marks,mark=o,mark size=1,mark repeat=2]table {Figures/PSD/TheoreticalVsWelch/PSMonteCarloDataSF7NQ2.dat};
\addlegendentry{Monte Carlo};

%\addplot[blue!60!white,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/fading_distance/SERMCMLr1.dat};
%\addlegendentry{$r_\mathrm{t}=1$ \ MC}
%
%\addplot[blue!60!white,only marks,mark=asterisk,mark size=3,mark repeat=4] table {Figures/fading_distance/SERAPPlowMLr1.dat};
%\addlegendentry{$r_\mathrm{t}=1$ \ APP (\ref{eq:avgSERfadinglow})}
%\addplot[blue!60!white,only marks,mark=square,mark size=3,mark repeat=4] table {Figures/fading_distance/SERAPPupMLr1.dat};
%\addlegendentry{$r_\mathrm{t}=1$ \ APP (\ref{eq:avgSERfadingup})}
%
%\addplot[green!60!black,solid] table {Figures/fading_distance/SERNumMLr4.dat};
%\addlegendentry{$r_\mathrm{t}=4$ \ Num}
%
%\addplot[green!60!black,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/fading_distance/SERMCMLr4.dat};
%\addlegendentry{$r_\mathrm{t}=4$ \ MC}
%\addplot[green!60!black,only marks,mark=asterisk,mark size=3,mark repeat=4] table {Figures/fading_distance/SERAPPlowMLr4.dat};
%\addlegendentry{$r_\mathrm{t}=4$ \ APP (\ref{eq:avgSERfadinglow})}
%\addplot[green!60!black,only marks,mark=square,mark size=3,mark repeat=4] table {Figures/fading_distance/SERAPPupMLr4.dat};
%\addlegendentry{$r_\mathrm{t}=4$ \ APP (\ref{eq:avgSERfadingup})}
%\addplot[red!60!white,solid] table {Figures/fading_distance/SERNumMLr16.dat};
%\addlegendentry{$r_\mathrm{t}=16$ Num}
%\addplot[red!60!white,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/fading_distance/SERMCMLr16.dat};
%\addlegendentry{$r_\mathrm{t}=16$ MC}
%\addplot[red!60!white,only marks,mark=asterisk,mark size=3,mark repeat=4] table {Figures/fading_distance/SERAPPlowMLr16.dat};
%\addlegendentry{$r_\mathrm{t}=16$ APP (\ref{eq:avgSERfadinglow})}
%\addplot[red!60!white,only marks,mark=square,mark size=3,mark repeat=4] table {Figures/fading_distance/SERAPPupMLr16.dat};
%\addlegendentry{$r_\mathrm{t}=16$ APP (\ref{eq:avgSERfadingup})}

%\addplot[blue,dashed,mark=star] table {Figures/fading_distance/SERSF7MCML2.dat};

%\addplot[orange!20!brown,mark=diamond,dashed] table {Figures/Figure1/BERM2methodsecondapproach.dat};
%\addplot[black,mark=o,dashed,mark options=solid] table {Figures/Figure1/BERM2methodthirdapproach.dat};
%	\addplot[red,dashed,mark=square] table {crbNoLISa4.dat};

%		\addplot[blue,mark=star] table {crbLISa1.dat};
%	\addplot[orange!20!brown ,mark=diamond,mark repeat=1] table {crbLISa2.dat};
%	\addplot[black,mark=o,mark options=solid] table {crbLISa3.dat};
% 	\addplot[red,mark=square] table {crbLISa4.dat};
%	\addplot[red,mark=square,mark repeat=4,dashed,mark options=solid] table {TSBCIM4fadingM4.dat};
%	\addplot[orange,mark=triangle,mark options=solid,mark repeat=2] table {UniformSD5fadingM4.dat}; 
%\addplot[orange,mark=star,mark size=1.5,mark repeat=6] table {UniformBCIM6fadingM4.dat};
%\addplot[brown] table {CapacityLBfadingM4.dat};
%\addplot[gray] table {PSDCEXPSF7.dat};
%\addplot[black,thick,mark repeat=4,mark options=solid] table {TxRatefadingM4.dat};
%\addplot[gray!50!black,thick,mark=o,mark options=solid, mark size=3] coordinates {
%	(6.65,1.13)
%};

%\addplot[gray,thin] table {Figures/FigPSDContMatlab/FFTFigPSDContSF12.txt};
%%/tikz/thin (no value)
%/tikz/ultra thin (no value)
%/tikz/very thin (no value)
%/tikz/semithick (no value)
%/tikz/thick (no value)
%/tikz/very thick (no value)
%/tikz/ultra thick
\end{axis}
\end{tikzpicture}

==> Figures/SER_AWGN/Figure_SER_AWGN_2p.tex <==
\pgfplotsset{every axis/.append style={
		font=\footnotesize,
		line width=1pt,
		legend style={font=\footnotesize, at={(0.405,0.36)}},legend cell align=left,nodes={scale=0.62, transform shape}},
	% 	legend style={font=\footnotesize, at={(0.99,0.75)}}
} %
\pgfplotsset{compat=1.13}
	\begin{tikzpicture}%[trim axis right]%[trim axis left, trim axis right]
\begin{axis}[
ymode=log,
%axis
%loglog
%title=Exact Analysis of WCL,
%axis x line=bottom,
%yticklabel style = {font=\footnotesize,xshift=0.5ex},
%xticklabel style = {font=\footnotesize,yshift=0.5ex},
%ylabel style = {font=\huge},
%xlabel style = {font=\huge},
xlabel near ticks,
ylabel near ticks,
grid=both,%major,minor,both,none
xlabel={SNR},
ylabel={SER},
width=0.99\linewidth,%3.5in,
%	ytick={10,0,-10,-20,-30,-40},
%	x label style={at={(axis description cs:0.5,-0.07)},anchor=north},
%   y label style={at={(axis description cs:-0.11,.5)},rotate=0,anchor=south},
yticklabel style={/pgf/number format},
%axis y line=left,
width=0.99\linewidth,
%height=0.6\textwidth,
%	legend columns=2,	
%legend pos=south west
%legend entries={
%	$r_\mathrm{t}=1$ \ MC,
%	$r_\mathrm{t}=1$ \ App,
%	$r_\mathrm{t}=4$ \ Num,
%	$r_\mathrm{t}=4$ \ MC,
%	$r_\mathrm{t}=4$ \ App,
%	$r_\mathrm{t}=16$ Num,
%	$r_\mathrm{t}=16$ MC,
%	$r_\mathrm{t}=16$ App
%	},
% 	log ticks with fixed point, 
%	scale only axis,
%	restrict
	xmin= -20, xmax=-5,
	ymin=1e-4, ymax=1e0,
ylabel style={font=\Large},
xlabel style={font=\Large},
%minor y tick num=10,
]
%\node[anchor=west] (source) at (axis cs:18,7e-1){Tag moving closer to Tx/Rx};
%\node (destination) at (axis cs:12,1e-3){};
%\draw[->,violet](source)--(destination);
%\addplot[blue!60!white,solid] table {Figures/SER_AWGN/SERSF8NumML1.dat};
%\addlegendentry{$\mathrm{SF}=8$, ML Num}

\addplot[blue!60!white,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/SER_AWGN/SERSF8MCML1.dat};
\addlegendentry{$\mathrm{SF}=8$, ML MC}

\addplot[blue!60!white,solid] table {Figures/SER_AWGN/SERSF8AppML1.dat};
\addlegendentry{$\mathrm{SF}=8$, ML Approx. (\ref{eq:avgSERAWGN})}

%\addplot[red!60!white,dashed] table {Figures/SER_AWGN/SERSF8Numfft1.dat};
%\addlegendentry{$\mathrm{SF}=8$, FFT Num}

\addplot[red!60!white,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/SER_AWGN/SERSF8MCfft1.dat};
\addlegendentry{$\mathrm{SF}=8$, FFT MC}

\addplot[red!60!white,dashed] table {Figures/SER_AWGN/SERSF8Appfft1.dat};
\addlegendentry{$\mathrm{SF}=8$, FFT Approx. (\ref{eq:avgSERAWGN})}

%\addplot[green!60!black,solid] table {Figures/SER_AWGN/SERSF9NumML1.dat};
%\addlegendentry{$\mathrm{SF}=9$, ML Num}

\addplot[green!60!black,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/SER_AWGN/SERSF9MCML1.dat};
\addlegendentry{$\mathrm{SF}=9$, ML MC}

\addplot[green!60!black,solid] table {Figures/SER_AWGN/SERSF9AppML1.dat};
\addlegendentry{$\mathrm{SF}=9$, ML Approx. (\ref{eq:avgSERAWGN})}

%\addplot[orange,dashed] table {Figures/SER_AWGN/SERSF9Numfft1.dat};
%\addlegendentry{$\mathrm{SF}=9$, FFT Num}

\addplot[orange,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/SER_AWGN/SERSF9MCfft1.dat};
\addlegendentry{$\mathrm{SF}=9$, FFT MC}

\addplot[orange,dashed] table {Figures/SER_AWGN/SERSF9Appfft1.dat};
\addlegendentry{$\mathrm{SF}=9$, FFT Approx. (\ref{eq:avgSERAWGN})}

%\addplot[blue,dashed,mark=star] table {Figures/SER_AWGN/SERSF7MCML2.dat};

%\addplot[orange!20!brown,mark=diamond,dashed] table {Figures/Figure1/BERM2methodsecondapproach.dat};
%\addplot[black,mark=o,dashed,mark options=solid] table {Figures/Figure1/BERM2methodthirdapproach.dat};
%	\addplot[red,dashed,mark=square] table {crbNoLISa4.dat};

%		\addplot[blue,mark=star] table {crbLISa1.dat};
%	\addplot[orange!20!brown ,mark=diamond,mark repeat=1] table {crbLISa2.dat};
%	\addplot[black,mark=o,mark options=solid] table {crbLISa3.dat};
% 	\addplot[red,mark=square] table {crbLISa4.dat};
%	\addplot[red,mark=square,mark repeat=4,dashed,mark options=solid] table {TSBCIM4fadingM4.dat};
%	\addplot[orange,mark=triangle,mark options=solid,mark repeat=2] table {UniformSD5fadingM4.dat}; 
%\addplot[orange,mark=star,mark size=1.5,mark repeat=6] table {UniformBCIM6fadingM4.dat};
%\addplot[brown] table {CapacityLBfadingM4.dat};
%\addplot[gray] table {PSDCEXPSF7.dat};
%\addplot[black,thick,mark repeat=4,mark options=solid] table {TxRatefadingM4.dat};
%\addplot[gray!50!black,thick,mark=o,mark options=solid, mark size=3] coordinates {
%	(6.65,1.13)
%};

%\addplot[gray,thin] table {Figures/FigPSDContMatlab/FFTFigPSDContSF12.txt};
%%/tikz/thin (no value)
%/tikz/ultra thin (no value)
%/tikz/very thin (no value)
%/tikz/semithick (no value)
%/tikz/thick (no value)
%/tikz/very thick (no value)
%/tikz/ultra thick
\end{axis}
\end{tikzpicture}

==> Figures/SER_AWGN/Figure_SER_AWGN_8p.tex <==
\pgfplotsset{every axis/.append style={
		font=\footnotesize,
		line width=1pt,
		legend style={font=\footnotesize, at={(0.405,0.36)}},legend cell align=left,nodes={scale=0.62, transform shape}},
	% 	legend style={font=\footnotesize, at={(0.99,0.75)}}
} %
\pgfplotsset{compat=1.13}
	\begin{tikzpicture}%[trim axis right]%[trim axis left, trim axis right]
\begin{axis}[
ymode=log,
%axis
%loglog
%title=Exact Analysis of WCL,
%axis x line=bottom,
%yticklabel style = {font=\footnotesize,xshift=0.5ex},
%xticklabel style = {font=\footnotesize,yshift=0.5ex},
%ylabel style = {font=\huge},
%xlabel style = {font=\huge},
xlabel near ticks,
ylabel near ticks,
grid=both,%major,minor,both,none
xlabel={SNR},
ylabel={SER},
width=0.99\linewidth,%3.5in,
%	ytick={10,0,-10,-20,-30,-40},
%	x label style={at={(axis description cs:0.5,-0.07)},anchor=north},
%   y label style={at={(axis description cs:-0.11,.5)},rotate=0,anchor=south},
yticklabel style={/pgf/number format},
%axis y line=left,
width=0.99\linewidth,
%height=0.6\textwidth,
%	legend columns=2,	
%legend pos=south west
%legend entries={
%	$r_\mathrm{t}=1$ \ MC,
%	$r_\mathrm{t}=1$ \ App,
%	$r_\mathrm{t}=4$ \ Num,
%	$r_\mathrm{t}=4$ \ MC,
%	$r_\mathrm{t}=4$ \ App,
%	$r_\mathrm{t}=16$ Num,
%	$r_\mathrm{t}=16$ MC,
%	$r_\mathrm{t}=16$ App
%	},
% 	log ticks with fixed point, 
%	scale only axis,
%	restrict
	xmin= -20, xmax=-8,
	ymin=1e-4, ymax=1e0,
ylabel style={font=\Large},
xlabel style={font=\Large},
%minor y tick num=10,
]
%\node[anchor=west] (source) at (axis cs:18,7e-1){Tag moving closer to Tx/Rx};
%\node (destination) at (axis cs:12,1e-3){};
%\draw[->,violet](source)--(destination);
%\addplot[blue!60!white,solid] table {Figures/SER_AWGN/SERSF8NumML3.dat};
%\addlegendentry{$\mathrm{SF}=8$, ML Num}

\addplot[blue!60!white,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/SER_AWGN/SERSF8MCML3.dat};
\addlegendentry{$\mathrm{SF}=8$, ML MC}

\addplot[blue!60!white,solid] table {Figures/SER_AWGN/SERSF8AppML3.dat};
\addlegendentry{$\mathrm{SF}=8$, ML Approx. (\ref{eq:avgSERAWGN})}

%\addplot[red!60!white,dashed] table {Figures/SER_AWGN/SERSF8Numfft3.dat};
%\addlegendentry{$\mathrm{SF}=8$, FFT Num}

\addplot[red!60!white,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/SER_AWGN/SERSF8MCfft3.dat};
\addlegendentry{$\mathrm{SF}=8$, FFT MC}

\addplot[red!60!white,dashed] table {Figures/SER_AWGN/SERSF8Appfft3.dat};
\addlegendentry{$\mathrm{SF}=8$, FFT Approx. (\ref{eq:avgSERAWGN})}

%\addplot[green!60!black,solid] table {Figures/SER_AWGN/SERSF9NumML3.dat};
%\addlegendentry{$\mathrm{SF}=9$, ML Num}

\addplot[green!60!black,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/SER_AWGN/SERSF9MCML3.dat};
\addlegendentry{$\mathrm{SF}=9$, ML MC}

\addplot[green!60!black,solid] table {Figures/SER_AWGN/SERSF9AppML3.dat};
\addlegendentry{$\mathrm{SF}=9$, ML Approx. (\ref{eq:avgSERAWGN})}

%\addplot[orange,dashed] table {Figures/SER_AWGN/SERSF9Numfft3.dat};
%\addlegendentry{$\mathrm{SF}=9$, FFT Num}

\addplot[orange,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/SER_AWGN/SERSF9MCfft3.dat};
\addlegendentry{$\mathrm{SF}=9$, FFT MC}

\addplot[orange,dashed] table {Figures/SER_AWGN/SERSF9Appfft3.dat};
\addlegendentry{$\mathrm{SF}=9$, FFT Approx. (\ref{eq:avgSERAWGN})}

%\addplot[blue,dashed,mark=star] table {Figures/SER_AWGN/SERSF7MCML2.dat};

%\addplot[orange!20!brown,mark=diamond,dashed] table {Figures/Figure1/BERM2methodsecondapproach.dat};
%\addplot[black,mark=o,dashed,mark options=solid] table {Figures/Figure1/BERM2methodthirdapproach.dat};
%	\addplot[red,dashed,mark=square] table {crbNoLISa4.dat};

%		\addplot[blue,mark=star] table {crbLISa1.dat};
%	\addplot[orange!20!brown ,mark=diamond,mark repeat=1] table {crbLISa2.dat};
%	\addplot[black,mark=o,mark options=solid] table {crbLISa3.dat};
% 	\addplot[red,mark=square] table {crbLISa4.dat};
%	\addplot[red,mark=square,mark repeat=4,dashed,mark options=solid] table {TSBCIM4fadingM4.dat};
%	\addplot[orange,mark=triangle,mark options=solid,mark repeat=2] table {UniformSD5fadingM4.dat}; 
%\addplot[orange,mark=star,mark size=1.5,mark repeat=6] table {UniformBCIM6fadingM4.dat};
%\addplot[brown] table {CapacityLBfadingM4.dat};
%\addplot[gray] table {PSDCEXPSF7.dat};
%\addplot[black,thick,mark repeat=4,mark options=solid] table {TxRatefadingM4.dat};
%\addplot[gray!50!black,thick,mark=o,mark options=solid, mark size=3] coordinates {
%	(6.65,1.13)
%};

%\addplot[gray,thin] table {Figures/FigPSDContMatlab/FFTFigPSDContSF12.txt};
%%/tikz/thin (no value)
%/tikz/ultra thin (no value)
%/tikz/very thin (no value)
%/tikz/semithick (no value)
%/tikz/thick (no value)
%/tikz/very thick (no value)
%/tikz/ultra thick
\end{axis}
\end{tikzpicture}

==> Figures/colormap/Figure_ColorMapLoRa.tex <==
\pgfplotsset{every axis/.append style={
		font=\footnotesize,
		line width=1pt,
		legend style={font=\footnotesize, at={(0.99,0.99)}},legend cell align=left,nodes={scale=1, transform shape}},
	% 	legend style={font=\footnotesize, at={(0.99,0.75)}}
} %
\pgfplotsset{compat=1.3}
	\begin{tikzpicture}%[trim axis right]%[trim axis left, trim axis right]
\begin{axis}[colorbar,
	view={0}{90},
%ymode=log,
%axis
%loglog
%title=Exact Analysis of WCL,
%axis x line=bottom,
%yticklabel style = {font=\footnotesize,xshift=0.5ex},
%xticklabel style = {font=\footnotesize,yshift=0.5ex},
%ylabel style = {font=\huge},
%xlabel style = {font=\huge},
%xlabel near ticks,
%ylabel near ticks,
%grid=both,%major,minor,both,none
%xlabel={$t$},
%ylabel={$\widetilde{Q}_N\off{f\of{t}}*\pi$},
%width=0.99\linewidth,%3.5in,
%	ytick={-1, -0.5,0,0.5,1},
%	yticklabels={$-\pi$,$-\frac{\pi}{2}$,$0$,$\frac{\pi}{2}$,$\pi$},
%	xtick={ 0,0.76393202,2,	4,	5.2360680,6,6.6055513,7.3944487,8},
%	xticklabels={$t_0$,$t_1$,$t_2$,$t_3$,$t_4$,$t_5$,$t_6$,$t_7$,$t_\psi$},
%	x label style={at={(axis description cs:0.5,-0.07)},anchor=north},
%   y label style={at={(axis description cs:-0.11,.5)},rotate=0,anchor=south},
%yticklabel style={/pgf/number format},
%axis y line=left,
width=0.99\linewidth,
%height=0.6\textwidth,
%	legend columns=3,	
%legend pos=south west
%legend entries={
%	$r_\mathrm{t}=1$ \ MC,
%	$r_\mathrm{t}=1$ \ App,
%	$r_\mathrm{t}=4$ \ Num,
%	$r_\mathrm{t}=4$ \ MC,
%	$r_\mathrm{t}=4$ \ App,
%	$r_\mathrm{t}=16$ Num,
%	$r_\mathrm{t}=16$ MC,
%	$r_\mathrm{t}=16$ App
%	},
% 	log ticks with fixed point, 
%	scale only axis,
%	restrict
%	xmin= 0, xmax=8,
%	ymin=-1, ymax=1,
%ylabel style={font=\large},
%xlabel style={font=\Large},
%minor y tick num=10,
]
%\node[anchor=west] (source) at (axis cs:18,7e-1){Tag moving closer to Tx/Rx};
%\node (destination) at (axis cs:12,1e-3){};
%\draw[->](source)--(destination);
%\addplot[blue!60!white,solid] table {Figures/fading_distance/SERNumMLr1.dat};
%\addlegendentry{$r_\mathrm{t}=1$ \ Num}
\addplot3[surf,only marks,scatter, mark=square]table {Figures/colormap/ColorMapDataLoRaSF6.dat};
%\addlegendentry{\acl{LB} $N=2$};

%\addplot[red!70!white]table {Figures/PSD/PowerSpectrum/PSDataSF9NQ3.dat};
%\addlegendentry{\acl{LB} $N=3$};
%
%\addplot[orange!70!white]table {Figures/PSD/PowerSpectrum/PSDataSF9NQ4.dat};
%\addlegendentry{\acl{LB} $N=4$};
%
%\addplot[purple!70!white]table {Figures/PSD/PowerSpectrum/PSDataSF9NQ5.dat};
%\addlegendentry{\acl{LB} $N=5$};
%
%\addplot[green!70!white]table {Figures/PSD/PowerSpectrum/PSMonteCarloDataSF9LoRa.dat};
%\addlegendentry{Normal LoRa};

%\addplot[blue!60!white,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/fading_distance/SERMCMLr1.dat};
%\addlegendentry{$r_\mathrm{t}=1$ \ MC}
%
%\addplot[blue!60!white,only marks,mark=asterisk,mark size=3,mark repeat=4] table {Figures/fading_distance/SERAPPlowMLr1.dat};
%\addlegendentry{$r_\mathrm{t}=1$ \ APP (\ref{eq:avgSERfadinglow})}
%\addplot[blue!60!white,only marks,mark=square,mark size=3,mark repeat=4] table {Figures/fading_distance/SERAPPupMLr1.dat};
%\addlegendentry{$r_\mathrm{t}=1$ \ APP (\ref{eq:avgSERfadingup})}
%
%\addplot[green!60!black,solid] table {Figures/fading_distance/SERNumMLr4.dat};
%\addlegendentry{$r_\mathrm{t}=4$ \ Num}
%
%\addplot[green!60!black,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/fading_distance/SERMCMLr4.dat};
%\addlegendentry{$r_\mathrm{t}=4$ \ MC}
%\addplot[green!60!black,only marks,mark=asterisk,mark size=3,mark repeat=4] table {Figures/fading_distance/SERAPPlowMLr4.dat};
%\addlegendentry{$r_\mathrm{t}=4$ \ APP (\ref{eq:avgSERfadinglow})}
%\addplot[green!60!black,only marks,mark=square,mark size=3,mark repeat=4] table {Figures/fading_distance/SERAPPupMLr4.dat};
%\addlegendentry{$r_\mathrm{t}=4$ \ APP (\ref{eq:avgSERfadingup})}
%\addplot[red!60!white,solid] table {Figures/fading_distance/SERNumMLr16.dat};
%\addlegendentry{$r_\mathrm{t}=16$ Num}
%\addplot[red!60!white,only marks,mark=o,mark size=3,mark repeat=4] table {Figures/fading_distance/SERMCMLr16.dat};
%\addlegendentry{$r_\mathrm{t}=16$ MC}
%\addplot[red!60!white,only marks,mark=asterisk,mark size=3,mark repeat=4] table {Figures/fading_distance/SERAPPlowMLr16.dat};
%\addlegendentry{$r_\mathrm{t}=16$ APP (\ref{eq:avgSERfadinglow})}
%\addplot[red!60!white,only marks,mark=square,mark size=3,mark repeat=4] table {Figures/fading_distance/SERAPPupMLr16.dat};
%\addlegendentry{$r_\mathrm{t}=16$ APP (\ref{eq:avgSERfadingup})}

%\addplot[blue,dashed,mark=star] table {Figures/fading_distance/SERSF7MCML2.dat};

%\addplot[orange!20!brown,mark=diamond,dashed] table {Figures/Figure1/BERM2methodsecondapproach.dat};
%\addplot[black,mark=o,dashed,mark options=solid] table {Figures/Figure1/BERM2methodthirdapproach.dat};
%	\addplot[red,dashed,mark=square] table {crbNoLISa4.dat};

%		\addplot[blue,mark=star] table {crbLISa1.dat};
%	\addplot[orange!20!brown ,mark=diamond,mark repeat=1] table {crbLISa2.dat};
%	\addplot[black,mark=o,mark options=solid] table {crbLISa3.dat};
% 	\addplot[red,mark=square] table {crbLISa4.dat};
%	\addplot[red,mark=square,mark repeat=4,dashed,mark options=solid] table {TSBCIM4fadingM4.dat};
%	\addplot[orange,mark=triangle,mark options=solid,mark repeat=2] table {UniformSD5fadingM4.dat}; 
%\addplot[orange,mark=star,mark size=1.5,mark repeat=6] table {UniformBCIM6fadingM4.dat};
%\addplot[brown] table {CapacityLBfadingM4.dat};
%\addplot[gray] table {PSDCEXPSF7.dat};
%\addplot[black,thick,mark repeat=4,mark options=solid] table {TxRatefadingM4.dat};
%\addplot[gray!50!black,thick,mark=o,mark options=solid, mark size=3] coordinates {
%	(6.65,1.13)
%};

%\addplot[gray,thin] table {Figures/FigPSDContMatlab/FFTFigPSDContSF12.txt};
%%/tikz/thin (no value)
%/tikz/ultra thin (no value)
%/tikz/very thin (no value)
%/tikz/semithick (no value)
%/tikz/thick (no value)
%/tikz/very thick (no value)
%/tikz/ultra thick
\end{axis}
\end{tikzpicture}

==> MyDefinitions.tex <==

%%%%%%%%%%%%% Manuscipt related %%%%%%%%%%%%%%%%%
%\def\scheme{\textit{\ac{DFTC} }} 
\def\scheme{\textit{\ac{SIDCo} }} %scheme name
\def\d{d} %Gradient length
\def\k{k} %number of elements to send
 \newcommand{\topk}{{\text{Top}_{\k}}} %The Sparse Source random variable
 \newcommand{\randk}{{\text{Rand}_{\k}}} %The Sparse Source random variable

\def\N{N}  % number of workers in a distributed setting
\def\x{\mathbf x}
%\def\xi [#1]{\x_{\{#1\}}}
\def\xin[#1]{{\x}_{\{#1\}}^{n}}
\def\gr{g} %realization for the gradient random variable
\def\g{\mathbf \gr}
\def\gin [#1]{{\g}_{#1}^{n}}
\def\G{G} %  gradient random variable
\def\C{\mathbb{C}_{\k}} % Compressor, the mapper 
\def\Tk[#1]{{\mathbb{T}}_{\k}\left\{ #1 \right\} } % Tok k tmapper 
\def\Ceta{\mathbb{C}_{\eta}} % Compressor, the mapper 
\def\sigmak{\sigma_{\k}}  % best k approximation
\def\p{p} % power law exponent
%%% distirbution parameters
\def\b{\beta} %scale parameters
\def\a{\alpha} %shape parameter
\def\loc{a}
\def\bhat{\hat{\beta}} %scale parameters
\def\ahat{\hat{\alpha}} %shape parameter
\def\lochat{\hat{a}}
%\alpha shape parameter







%%%%%%%%%%%%%% Math %%%%%%%%%%
\def\sign{\textrm{sign}}                                              % Sign function
\def\erf{\textrm{erf}}
\def\erfc{\textrm{erfc}}

% Hypothesis testing
\def\Hzero{{{\mathcal{H}}_{0}}}
\def\Hone{{{\mathcal{H}}_{1}}}
\def\Hl{{{\mathcal{H}}_{l}}}

\def\Dzero{{{\mathcal{D}}_{0}}}
\def\Done{{{\mathcal{D}}_{1}}}

\def\testH1overH0{\begin{array}{l}
		{\mathcal{H}}_1 \\
		\gtrless \\
		{\mathcal{H}}_0
\end{array}}

\def\testH0overH1{\begin{array}{l}
		{\mathcal{H}}_0 \\
		\gtrless \\
		{\mathcal{H}}_1
\end{array}}

\def\testD1overD0{{ \begin{array}{l}
			{\mathcal{D}}_1 \\
			\gtrless \\
			{\mathcal{D}}_0
\end{array}}}





